Empirical Evaluation of Ambient Sensors as Proximity Detection Mechanism for Mobile Payments

Near Field Communication (NFC) has enabled mobile phones to emulate contactless smart cards. Similar to contactless smart cards, they are also susceptible to relay attacks. To counter these, a number of methods have been proposed that rely primarily on ambient sensors as a proximity detection mechanism (also known as an anti-relay mechanism). In this paper, we, for the first time in academic literature, empirically evaluate a comprehensive set of ambient sensors for their effectiveness as a proximity detection mechanism. We selected 15 out of a total of 17 sensors available via the Google Android platform for evaluation, with the other two sensors unavailable on widely-used handsets. In existing academic literature, only 5 sensors have been proposed with positive results as a potential proximity detection mechanism. Each sensor, where feasible, was used to record the measurements of 1000 contactless transactions at four different physical locations. A total of 252 random users, random sample of the university student population, were involved during the field trails. The analysis of these transactions provides an empirical foundation to categorically answer whether ambient sensors provide a strong proximity detection mechanism for security sensitive applications like banking, transport and high-security access control. After careful analysis, we conclude that no single evaluated mobile ambient sensor is suitable for such critical applications in realistic deployment scenarios. Lastly, we identify a number of potential avenues that may improve their effectiveness.

==> sections/ambient_sensors.tex <==
\section{Ambient Sensor Deployment in Mobile Payment}
\label{sec:AmbientSensorDeploymetinMobilePayment}
In this section, to set the scenery, we briefly describe the contactless payments (both smart card and mobile), relay attacks and framework to deploy ambient sensors as anti-relay mechanism. 

\subsection{Contactless Mobile Handsets and Relay Attacks}
\label{sub:ContactlessMobileHandsetsAndRelayAttacks}
In a contactless transaction whether it is a payment, transport or access control etc.\ the overall architecture and process is the same. The only difference is in the higher level protocol that implements the semantic of each of the applications. Therefore, in this section we deal with the contactless transaction as a mobile payment; however, the overall architecture is common across all deployment applications. 

When a user brings her NFC enabled mobile phone close to a contactless payment terminal. The NFC in the mobile handset enters the range of a RFID (Radio Frequency Identification) around a payment terminal, it can initiate a dialog with the terminal. This dialog contains the specific protocol messages required for a successful completion of the transaction. As a physical contact is not necessary and in some case there is no second factor authentication like biometrics or PIN (Personal Identification Number), it is difficult to ascertain whether the genuine user was the one that brought the mobile phone near the terminal. 

\begin{figure}[ht]
	\centering
		\includegraphics[width=0.95\columnwidth]{images/Relay_Attacks.png}
	\caption{Generic Overview of a Relay Attack}
	\label{fig:relay_attack}
\end{figure}

In a relay attack as shown in figure \ref{fig:relay_attack}, an attacker has to emulate a malicious terminal to a genuine user and a masquerading payment instrument (mobile phone) to a genuine terminal. The objective of the malicious user to extend the communication between the genuine user's mobile phone and the payment terminal -- relaying each messages across the (extended) distance. If the malicious user relays the message in a manner that both the payment terminal and user's mobile phone do not detect that the messages are relayed, the attacker might be able to pay for services via genuine user's account. 

In the contactless smart card deployment, the problem of relay attack is resolved using distance bounding protocols \cite{rasmussen2010realization} or their variants \cite{Hancke2009615}. The relay attacks on contactless smart cards and their countermeasures is still an active domain with new attacks and countermeasures emerging \cite{hancke2008attacks,Cremers2012,boureanu2014towards}. The main objective of the distance bounding protocols is to facilitate a terminal (verifiers) to enforce an upper bound on its physical distance to a smart card (prover). This enforcement of physical distance is achieved by  periodic challenge-response exchange and timing it. If the response is received within a predefined time the verifiers ascertains that the prover is within specified physical distance. In a relay attack, we can have provers to be either malicious or genuine, however, we considered verifiers to be honest as if they are malicious and try to participate in a relay attack then in fact they are attacking themselves. This defeats the purpose of such an attack. 

In the domain of the contactless mobile transactions via NFC, to provide a notion of proximity a number of proposals are based on environmental (ambient) sensors present on these mobile handsets (for related work discussion see section \ref{sec:RelatedWork}). In the subsequent section, we discussion how these ambient sensors are proposed to counter the relay attacks in NFC based mobile (contactless) transactions. 


\subsection{Ambient Sensors as Proximity Detection Mechanism}
An ambient sensors detects different elements of the environment in immediate surroundings for example, temperature, light, gravity and sound etc. Most of the smart phones now a days are equipped with one or more of these sensors. The physical environment surrounding a smart phone (or a terminal) can provide a rich set of attributes that might be unique for example sound and light to a particular location. Therefore, such an information might be useful to create a contextual environment in which two devices interacted with each other and can be used to facilitate the proximity detection. 

\begin{figure}[ht]
	\centering
		\includegraphics[width=0.95\columnwidth]{images/AmbientSensorAntiRelay.png}
	\caption{Generic Deployments of Ambient Sensors as Proximity Detection Mechanism}
	\label{fig:AmbientSensorDeploymentOverview}
\end{figure}

In this section, we illustrate a generic framework put forward about the deployment of ambient sensors as proximity detection mechanism especially in the context of mobile payments. Figure \ref{fig:AmbientSensorDeploymentOverview} illustrates variants of proximity detection frameworks based on the ambient sensors, which are listed as below.

\begin{enumerate}
\item Independent Reporting: In this deployment scenario, also depicted as solid lines in the figure \ref{fig:AmbientSensorDeploymentOverview}, both the smart phone and terminal perform sensor measurements independent of each other and then sends them to a trust authority. This authority then compares the sensor measurements, based on some predefined comparison algorithm with set margin for errors, it decides whether the two devices where in proximity to each other or not. 
\item Terminal Dependent Reporting: This scenario is depicted as double-dot-dash line in the figure \ref{fig:AmbientSensorDeploymentOverview} and in this deployment the smart phone encrypts the sensor measurement with a shared key (between smart phone and trusted authority) and gives this encrypted message to the terminal. That then sends smart phone's and its own measurements to the trusted authority for comparison. 
\item Terminal (Localised) Evaluation: In this scenario, the smart card provides its own measurement to the terminal that then locally compares it with its own measurements. The decision is taken by the terminal whether the smart phone is in its proximity or not. 
\end{enumerate}

Whether a user does a single tab on the terminal or multiple tabs with his or her smart phone. The overall deployment architecture falls under one of the above three scenarios. It can be observed that there is a potential for a fourth scenario to have a mobile phone perform the proximity analysis, however, as we consider the terminal to be the (potentially) trusted device as per discussion in section \ref{sub:ContactlessMobileHandsetsAndRelayAttacks}.


\subsection{Related Work}
\label{sec:RelatedWork}
A large portion of the work about anti-relay countermeasures for the contactless smart cards was mainly around distance bounding protocols \cite{DrimerM07,Francillon11} as discussed before. However, they at the current state-of-the-art might not be feasible for the NFC phones because of their requirement of high time-delay sensitivity and special-purpose hardware \cite{Coskun2013,Halevi2012}.  

Drimer et al. \cite{DrimerM07} and Ma et al. \cite{ma2013location} showed how the location related data (GPS: Global Positioning System) can be used as an ambient sensor to ascertain the proximity of two NFC mobile phones. Ma used ten seconds sample where collecting the location information at each second. The collected GPS information was the compared across different devices and as per the paper they had a high success rate in identify the devices that were in close proximity to each other. 

Halevi et al. \cite{Halevi2012} demonstrated the applicability of the audio (sound) sensor and ambient light sensor. In this paper they analyised the data using various algorithms and performed extensive experiments to provide a success rate --- approaching 100\% detection rate. 

Varshavsky et al. \cite{Varshavsky2007} based their proximity detection mechanism on the radio channels like WiFi access points, cell phones, and Bluetooth. In this paper they only evaluated the WiFi and considered it have low error rate, recommending it as a the proximity detection mechanism. However, there paper did not focused on NFC mobile transactions but their results might still be applied to the requirement of proximity detection in such transactions. 

Urien et al \cite{Urien201428} selected the temperature as the sensors choice to provide an anti-relay mechanisms. They combined the temperature sensors with Elliptic curve-based RFID/NFC authentication protocol to demonstrate the devices where in close proximity to each other and were successful in establishing a secure channel. The proposal mixed the timing channels in the RFID (traditionally used by distance bounding protocol) and ambient sensors (temperature); however, their paper do not demonstrate the proposal being practical for NFC mobile phones. Furthermore, there is no experimental data provided to ascertain the success rate. 

Mehrnezhad et al. \cite{mehrnezhad2014tap} proposed the use of accelerometer to provide the assurance that the payment mobile phone is in proximity of the terminal. Their proposal requires double tap, the user has to present his or her mobile phone twice to the terminal and one each time they have to tap the terminal. Although, it is difficult to deduce the total time it took to complete one transaction but authors have provided a recording time range of 0.6 and 1.5 seconds. 

  \begin{table}[ht]
	\centering
	\caption{Related Work in Sensors as Anti-Relay Mechanism}
	\label{tab:RelatedWork}
    \resizebox{\columnwidth}{!}{
\def\arraystretch{1.2}
			\begin{tabular}{@{}lccc@{}}
				\toprule
				\multirow{2}{*}{\textbf{Paper}} & \multirow{2}{*}{\textbf{Sensor}} 
                & \textbf{Sample} & \textbf{Contactless}\\
                && \textbf{Duration} & \textbf{Applicability}\\
                \midrule
    	 Ma et al.  \cite{6378376} & GPS & 10 seconds & May be Not \\ [0.6ex]
         \hdashline 
        \multirow{2}{*}{Halevi et al. \cite{Halevi2012}} & Audio  & 30 seconds &  May be Not\\ 
        												 & Light  & 2 seconds &  Potentially \\ [0.8ex]
                                                         \hdashline
      	\multirow{2}{*}{Varshavsky et al. \cite{Varshavsky2007}} & WiFi & \multirow{2}{*}{1 second} & \multirow{2}{*}{Potentially} \\ 
        													     & (Radio Waves) &  &  \\ [0.6ex]
                                                                 \hdashline
    	Urien et al. \cite{Urien201428} & Temperature & N/A & - \\ [0.6ex]
        \hdashline
        Mehrnezhad et al. \cite{mehrnezhad2014tap} & Accelerometer & 0.6 to 1.5 Seconds & Potentially\\
    
		\bottomrule
			\end{tabular}
    }
\end{table}

We have summerised the related work in the table \ref{tab:RelatedWork} with sensor sample time and whether the proposed time is suitable for a contactless NFC mobile phone services like banking, transport and access control. Ambient sensors are also used in the traditional user authentication, key generation and establishment of secure channels. As these application might not requires a high granularity of proximity (with in few centimeters) we do not discuss them in this section. The field of ambient sensors for proximity detection for NFC mobile services is developing and as shown in this section, there are proposals around to use some of the ambient sensors to achieve this. In this paper, we extend the discussion of a large set of ambient sensors -- some are already considered as proximity evidence where others are not yet proposed. In a way, this paper not only evaluated the validity of different ambient sensors as a proximity evidence but also experimented with sensors that are not proposed in literature as anti-relay mechanisms for NFC mobile phones. Table \ref{tab:availability} shows that we have a detailed evaluation of fifteen sensors out of which only five are proposed for proximity detection in existing literature, effectively testing the applicability of additional ten sensors for anti-relay mechanism.  




==> sections/conclusion.tex <==
\section{Conclusion}
%\todo[linecolor=green!90!white, backgroundcolor=purple!20!white,
 %bordercolor=red, inline]{Mainly written by Raja}
 
The objective of the paper was to evaluated and analyse different sensors present in modern day mobile phones -- ascertaining which of them would be suitable to the application of proximity detection in the specific domain of NFC phone transactions (e.g. banking, transport and access control etc.). We shortlisted 17 sensors documented to be available on Google Android handsets. However, only 15 of them are widely deployed; therefore, we limited out analysis to these sensors. It has to be noted that in the existing literature only five of these fifteen sensors are proposed to be used a proximity detection mechanism. In this paper, we are extending this with ten additional sensors by implementing them to evaluate their validity and effectiveness as a proximity detection mechanism to be deployed in NFC mobile phones. Our analysis of these sensors were scoped to NFC mobile phones that emulate traditional smart card services like banking, transport and access control. 

The experimentation and analysis carried out part of this paper showed that {\tt{XX}} number of sensors including {\tt{ABC}}, {\tt{EYJ}}, and {\tt{XUD}} can be deploy; however, before doing so the developer should take into account the associated risks. Furthermore, {\tt{YY}} number of the sensors in the set can be considered as not suitable for the proximity detection mechanisms. For each of the sensors we have provided an EER graph which clearly indicates the effectiveness of the respective sensor and associated risk if it to be deployed. From the data we have analysied we can safely claim that mobile sensors with their current state in most of the Google Android devices might not be suitable for deployment as a anti-relay mechanism. They might be suitable for a niche application with limited exposure of users, but for a large scale field deployment more evaluation and experimentation needs to be carried out. 

Furthermore, we will make source code for the test-bed and collected data-set open to public for open scrutiny and further analysis of experimented sensors. 

==> sections/evaluation.tex <==
\section{Ambient Sensor Evaluation}
\label{sec:AmbientSensorEvaluation}
%\todo[linecolor=green!90!white, backgroundcolor=purple!20!white,
% bordercolor=red, inline]{Mainly written by Raja... Iakovos \& Carlton to assist}

%\subsection{Individual Location Analysis of Data}

In this section, we will describe the methodology to calculate False Positive Rate (FPR), False Negative Rate (FNR) and Equal Error Rate (EER). Furthermore, this section also put forward results of experimentation for individual sensors.  

\subsection{Calculating the FPR, FNR and EER}
As discussed in the section \ref{sec:DataAnalysisandEvaluationCriteria}, each transaction generated a set of $R_i$ and $C_i$. From this (per transaction) data we then calculated the $MAE(R_i, C_i)$ and $corr(R_i, C_i)$ for each transaction. The data set consist of four values $R_i$, $C_i$, $MAE(R_i, C_i)$ and $corr(R_i, C_i)$ for each of the transaction. From these per transaction data set we then calculated the FPR, FNR and EER based on the $MAE$ and $corr$. to calculate the FPR we implemented the algorithm illustrated in listing \ref{CalculatingFAR}:

\begin{lstlisting}[style=customc, caption={Calculating False Positive Rate},label=CalculatingFAR]
/* Pseudocode to calculate FPR data points */
int maxint = Number_of_Transactions;
for (int i = 1; i <= maxint; i++) {
  int FPR = 0;
  for (int j = 1; j <= maxint; j++) {
    if (i != j) {
      calculateMAE(Ri, Cj);
      if (MAE(Ri, Cj) <= MAE(Ri, Ci))
        FPR++;
    }
  }
  write(MAE(Ri, Ci), FPR);
}
\end{lstlisting}

The calculation of FPR based on $corr$ follows the same algorithm, only substituting $MAE$ with transaction $corr$ values. To calculate the False Negative Rate (FNR) we implemented the algorithm illustrated in listing \ref{CalculatingFNR}. Similar to the calculation of FPR, in the listing \ref{CalculatingFNR} substitute $MAE$ with the $corr$ to generate the FPR curve (based on $corr$ calculations). 

\begin{lstlisting}[style=customc, caption={Calculating False Negative Rate},label=CalculatingFNR]
/* Pseudocode to calculate FNR data points */
int maxint = Number_of_Transactions;
for (int i = 1; i <= maxint; i++) {
  int FAR = 0;
  for (int j = 1; j <= maxint; j++) {
    if (i != j) {
      calculateMAE(Ri, Cj);
      if (MAE(Ri, Ci) < MAE(Rj, Cj)
        FNR++;
    }
  }
  write(MAE(Ri, Ci), FNR);
}
\end{lstlisting}

\subsection{Individual Sensor's Results}
The aim of our evaluation is investigate to what extent legitimate and illegitimate transactions can be identified using these similarity metrics.  Ideally, for a transaction between two co-located devices, then $MAE(R_{i}, C_{i}) \approx 0$ and $corr(R_{i}, C_{i}) \approx 1$, while for a card and reader in differing locations, i.e. $(R_{i}, C_{j})$, the distance and correlation should be sufficiently large.  What is considered `sufficient' is determined through finding a suitable threshold, $t$, which permits all legitimate transactions while denying those which are illegitimate, i.e. $similarity(R_{i}, C_{i}) < t$ and $similarity(R_{i}, C_{j}) > t$.  For each individual sensor, we aim to find an optimal value of $t$, along with its reliability.

\begin{figure}[ht]
	\centering
		\includegraphics[width=0.95\columnwidth]{images/EER_Accelerometer.png}
	\caption{FPR and FNR Graph for Accelerometer based on $MAE(R_i,C_i)$}
	\label{fig:EERAmbientSensor}
\end{figure}

Plotting the FPR and FNR curves for each of the matrix ($MAE$ and $corr$) for every sensors for which we were able to collect data. The point of intersections for these curves gave as the optimum threshold for $MAE$ and $corr$. Furthermore this intersection point also indicates the EER for the optimum threshold. Figure \ref{fig:EERAmbientSensor} shows the FPR and FNR curves for the accelerometer (based on $MAE$ calculations), along with the optimum threshold and EER\@. Appendix \ref{sec:AmbientSensors} includes the EER graphs for all of the tested sensors (except Accelerometer) -- based on both $MAE$ and $corr$ methods. 

The figure \ref{fig:EERAmbientSensor} clearly shows that the optimum threshold (based on the $MAE$) is at 0.651 with EER 0.506. These numbers describe that the best result you can except from an Accelerometer sensors (at least of the devices included in the experiments) at 0.651 threshold, but at this threshold approximately you will have 50\% {\tt{false positive}} and {\tt{false negatives}}. 

\begin{figure}[ht]
	\centering
		\includegraphics[width=0.95\columnwidth]{images/EER-Corr_Accelerometer_corr.png}
	\caption{FPR and FNR Graph for Accelerometer based on $corr(R_i,C_i)$}
	\label{fig:EERAmbientSensorcorr}
\end{figure}

Similarly, figure \ref{fig:EERAmbientSensorcorr} shows that at the optimum threshold of 0.007 the EER would be 0.523. Therefore, if we use the $corr$ as the comparison method we will have 50\% {\tt{false positive}} and {\tt{false negative.}}. Table \ref{tab:OptimumThresholds} lists the optimum thresholds and associated EER for each of the sensors. 

To enable a wide-scale deployment of the proximity detection mechanism based on mobile sensor data, we need to define an acceptable threshold. For example, a terminal can define a threshold and as long as the mobile phones sensor measurement is within the limits of this threshold it would accept it as a valid transaction (performed in proximity to the terminal). However, setting these threshold also incur the potential of {\tt{false positives}} and {\tt{false negatives}}. In intersection of the FPR and FNR provides us with the percentage of potentially malicious transactions might passing as genuine ({\tt{false positives}}) and genuine transactions being rejected ({\tt{false negatives}}). The objective of a malicious entity would be carry out the relay attacks in a manner that the sensor measurements carried out at the terminal and mobile phone remain within the set threshold -- thus successfully mounting the relay attack. A threshold with a higher rate of {\tt{false positives}} will give a large working space to the malicious entity. Whereas a higher rate of the {\tt{false negatives}} might make the scheme less user friendly. 

\begin{table}[ht]
	\centering
	\caption{Optimum Thresholds and Associated Risk for Each Sensors}
	\label{tab:OptimumThresholds}
	\resizebox{\columnwidth}{!}{
			\begin{tabular}{@{}lcccc@{}}
				\toprule
				\multirow{2}{*}{\textbf{Sensors}} & \textbf{Optimum} & \multirow{2}{*}{\textbf{$EER_{MAE}$}} & \textbf{Optimum} & \multirow{2}{*}{\textbf{$EER_{corr}$}} \\ 
                								  & \textbf{Threshold$_{MAE}$} & & \textbf{Threshold$_{corr}$}& \\
                                                  \midrule
				\textbf{Accelerometer} & 0.651 & 0.506 & 0.007 & 0.523 \\
				\textbf{Bluetooth} & -- & -- & -- & -- \\
				\textbf{GRV} & 0.499 & 0.615 & 0.006 & 0.518 \\
				\textbf{GPS} & -- & -- & -- & -- \\
				\textbf{Gyroscope} & 0.520 & 0.504 & 0.007 & 0.752 \\
				\textbf{Magnetic Field} & 77.33 & 0.334 & 0.235 & 0.582 \\
				\textbf{Network Location} & 8.532 & 0.369 & N/A\footnote{Insufficient data to calculate correlation} & N/A \\
				\textbf{Pressure} & 2.787 & 0.270 & 0.329 & 0.645 \\
				\textbf{Rotation Vector} & 1.4e19 & 0.635 & 0.979 & 0.885 \\
				\textbf{Sound} & \cmark & \cmark & \cmark & \cmark \\
				\textbf{WiFi} & -- & -- & -- & -- \\
				\textbf{Gravity} & 9.5e-05 & 0.506 & 0.020 & 0.534 \\
				\textbf{Light} & 176.6 & 0.507 & 0.007 & 0.510 \\
				\textbf{Linear Acceleration} & 1.348 & 0.514 & 0.087 & 0.491 \\
				\textbf{Proximity} & N/A\footnote{All transactions contained the same value for both devices.  Consequently, EER is undefined.} & N/A & N/A & N/A \\
				\bottomrule
			\end{tabular}
            }
\end{table}

Beside understanding their implication of the EER and thresholds on the suitability of a mobile sensor for the NFC mobile services. Further to this analysis, we also evaluated the usability and reliability of the selected sensors. This analysis is shown in table \ref{tab:UsabilityandReliability}.

\begin{table}[ht]
	\centering
	\caption{Usability and Reliability Analysis of Each Sensor}
	\label{tab:UsabilityandReliability}
	\resizebox{\columnwidth}{!}{
			\begin{tabular}{@{}lccc@{}}
				\toprule
				\multirow{2}{*}{\textbf{Sensors}} & \textbf{Total} &\textbf{Transaction} & \textbf{Sensor} \\ 
                                                  & \textbf{Transactions}& \textbf{Failures} &  \textbf{Failures}\\
                								  \midrule
				\textbf{Accelerometer} & 1025 & 13 & 0 \\
				\textbf{Bluetooth} & 101 & 1 & 100 \\
				\textbf{GRV} & 1019 & 8 & 0 \\
				\textbf{GPS} & 101 & 1 & 100 \\
				\textbf{Gyroscope} & 1022 & 11 & 0 \\
				\textbf{Magnetic Field} & 1027 & 17 & 0 \\
				\textbf{Network Location} & 1053 & 15 & 960 \\
				\textbf{Pressure} & 1018 & 10 & 0 \\
				\textbf{Rotation Vector} & 1023 & 14 & 0\\
				\textbf{Sound} & \cmark & \cmark & \cmark \\
				\textbf{WiFi} & 100 & 0 &  100\\
				\textbf{Gravity} & 1165 & 143 & 0\\
				\textbf{Light} & 1057 & 37 & 0\\
				\textbf{Linear Acceleration} & 1175 & 159 & 3 \\
				\textbf{Proximity} & 1071 & 58 & 0\\
				\bottomrule
			\end{tabular}
            }
\end{table}

To collect 1000 transactions from 252 users (for each sensor), we requested them to tab the mobile handset on to the terminal as many time as they prefer. During this process, some time a user tabs the mobile handset the transaction does not successfully complete (due to the user moving the mobile handset away too quickly). This is represented as the "Transaction's Failure in the table \ref{tab:UsabilityandReliability}. Whereas, the "Sensor's Failure" in the same table represent the situation when the transaction was successfully completed on both the terminal and mobile handset, but either both or one of them did not successfully measure the sensor data. The transactions failure represents the difficulty in using the sensors by the user, and the sensor's failure illustrates the reliability of the individual sensors. 

%\subsection{Putting Results into the Context}




==> sections/experiment.tex <==
\section{Experimentation and Challenges}
\label{sec:ExperimentationandChallenges}

%\todo[linecolor=green!60!white, backgroundcolor=blue!20!white,
 %bordercolor=red, inline]{Section is shared between Iakovos and Carlton}

%\rajaComment{In this section, different challenges faced during the development, experimentation and evaluation phases are discussed}

In this section, we discuss the challenges we had to overcome in order to implement the test-bed with individual sensors, issues with data collection and the evaluation of the collected data. 

==> sections/experiment_analysis.tex <==
\subsection{Data Analysis Challenges}



%\todo[linecolor=green!90!white, backgroundcolor=green!40!white,
 %bordercolor=red, inline]{Mainly written by Carlton... Iakovos to assist if required}
During the data collection in the field, we were faced a number of challenges. Below is a list of some selected challenges that we had to overcome. 

\begin{itemize}
\item After acquiring the data from the card and reader, we used linear interpolation to mitigate the effect of missing and inconsistent samples due to the unwanted variation in sampling rates (stages \textbf{1} and \textbf{2} of Figure \ref{fig:workflow}).

% \begin{figure*}
% \centering
% \includegraphics[width=\textwidth]{images/FlowsThreeGraph.pdf}
% \caption{Data analysis workflow for an accelerometer-based transaction}
% \label{fig:workflow}
% \end{figure*}

\item Data sampling rarely finished at 500ms precisely: Figure \ref{fig:magfield} illustrates that the reader's final sample occurs at $\approx$490ms, while the card finished at $\approx$460ms.  To counter this, interpolation was performed up to the maximum time period shared by both devices (460ms) and any samples beyond this point were discarded.  
	\begin{itemize}
    	\item Correlation, however, is sensitive to this type of truncation.  If relatively extreme values are discarded, such as the reader's measurements between 0-100ms in Figure \ref{fig:magfield}, then correlation may differ significantly.  
    \end{itemize}
\item Only one measurement was collected at maximum -- if any were collected at all -- when analysing network location for all transactions.  Since correlation is undefined for a single point, we calculated only the MAE for this particular modality.

\item For 42.5\% of gyroscope-based transactions (430 of 1011), a value of zero was measured for the entire transaction on the card or reader, indicating that the device was not perturbed sufficiently to alter the sensor's resting value.  As with before, correlation is undefined for a single point, so these transactions were discarded for the correlation analysis.

\item The proximity sensor on both tested device returned only a binary value, representing \emph{near} and \emph{far}, rather than the precise proximity of the device to an object in centimeters.  The Android documentation states that `some' devices provide a binary value rather than a real value \cite{androidposition}.  In our dataset, both devices registered as `far' for all transactions, as the proximity sensor -- located on the front of the device -- was not covered on either end.
\end{itemize}

\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{images/MagneticField.eps}
\caption{Example Magnetic Field transaction illustrating differing finishing times for the card and reader}
\label{fig:magfield}
\end{figure}



==> sections/experiment_implementation.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{images/Step_One1.png}
        \caption{Step One}
        \label{fig:Step_One}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{images/Step_Two.png}
        \caption{Step Two}
        \label{fig:Step_Two}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{images/Step_Three.png}
        \caption{Step Three}
        \label{fig:Step_Three}
    \end{subfigure}
    \caption{Data Analysis Workflow for an Accelerometer-based Transactions}\label{fig:workflow}
\end{figure*}

\subsection{Implementation Challenges}
\begin{itemize}
	\item The clocks of the two devices involved in a transaction cannot be expected to be completely synchronised, especially in a real-world scenario.
		In order for the measurements on the devices to begin as close to each other as possible, all the checks are being performed after the recordings have finished.
		In case of inconsistencies, the recorded measurement gets rejected.
	\item In order to capture the maximum possible amount of data, the code of the applications was designed so that no threads, or other process intense components are used, other than the ones automatically initiated by the Android API\@.
		The threads initiated by the Android API were responsible to listen for sensor changes.
	\item The sound recording sensor's development was extremely challenging.
		There are various ways to access the microphone on Android, as well as many settings for storing the actual recording.
		In most of the implementations, we were either not capable to initiate the microphone in the timeframe of 500ms, or an empty file was created.
		By setting the sample rate to 8kHz and saving the data in raw format, we achieved to record data in the specified timeframe, using the \texttt{AudioRecord} class.
	\item Ensuring that the recording of each sensor will not exceed 500ms since the initiation of the transaction was a big challenge.
		A common way to run a task for a specific amount of time in Java is by using a timer inside a thread.
		Since the timer is initiated after the creation of a thread, which is a processor intense procedure, there is no guarantee that the measurement will last for no more than 500ms since the initiation of the transaction. 
		To overcome this issue, we track the system time on the terminal side when it sends the first message to the device and on the mobile device side, when it receives the first message from the terminal.
		A loop ensures that measurements after the 500ms timeframe will not be stored and the recording will terminate.
	\item The \texttt{HostApduService} class was used for the implementation of the mobile device application, which is capable of emulating an NFC card on an Android handset, and is the basis of implementing a Host Card Emulation (HCE) service~\cite{hce}.
		HCE was introduced on Android 4.4 (API level 19), therefore the handset that acts as the mobile device in the experiment should be running Android 4.4 or later.
	\item The data from the sensors was retrieved in time intervals of 10ms.
		The SGS5 mini device was capable of collecting data at a higher frequency (less than 1ms), the fastest common value across all our devices was 10ms.
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Data Collection Challenges}

\begin{itemize}
	\item Although the sampling rate for retrieving sensor values was set to 10ms, we encountered variance in the intervals that sensors return data and granularity in the returned data, across different devices.
		There are various reasons why this may occur.
		Only when there is a change in the values recorded by a sensor, they are returned to an application~\cite{AndroidAPIRef}.
		Therefore, if over a period larger than 10ms there has been no change in the values observed by the sensor, no new data will be returned to an application.
		Other processes, services and daemons running on the background may also be causing slight delays to the frequency that an application is notified about sensor changes.
		During our experiments we ensured that delays due to that reason are limited to a minimum, by uninstalling applications that cause heavy CPU load and turning off all the synchronisation services.
	\item Various sensors were excluded from the study, since they were not capable of returning any useful data in the 500ms timeframe.
		These sensors are the WiFi, GPS and Bluetooth.
		The first 100 measurements that were performed included these sensors, but since no, or very little data was captured, they were excluded.
		A separate application was built in order to measure the actual time required for the WiFi and Bluetooth sensors in order to capture data.
		The GPS sensor's speed and accuracy are very dependant on the environment in which it is being tested.
		The results for 50 measurements are presented in table~\ref{tab:wifibt}.
		The results for the Bluetooth concern the time required to detect one device.
\end{itemize}

\begin{table}[ht]
	\centering
	\caption{Timing for getting results from sensors}
	\label{tab:wifibt}
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{@{}llll@{}}
			\toprule
			\multicolumn{1}{c}{\textbf{Sensor}} & \multicolumn{1}{c}{\textbf{Average time}} & \multicolumn{1}{c}{\textbf{Minimum time}} & \multicolumn{1}{c}{\textbf{Maximum time}} \\ \midrule
			\textbf{Bluetooth} & 962.7ms & 354ms & 1960ms \\
			\textbf{WiFi} & 3873.5ms & 3795ms & 3954ms \\ \bottomrule
		\end{tabular}
	}
\end{table}


==> sections/framework_part1.tex <==
\section{Framework for Evaluation of Ambient Sensors Effectiveness}
\label{sec:FrameworkforEvaluationofAmbientSensorsEffectiveness}

%todo write about the light sensor on tablets!

%\rajaComment{In this section, we will describe our test environment that we are going implement in order to gain empirical data for evaluation}
In this section, the test-bed that was developed in order to test, analyse and evaluate the effectiveness of using ambient sensors as an anti-relay mechanism is described.
The results of the evaluation are presented in section~\ref{sec:AmbientSensorEvaluation}.

\subsection{Evaluation Test-bed Architecture}
Two applications were built and installed on pairs of Android devices, one acting as the terminal and the other as the mobile device involved in the transaction.
When the two devices touch, an NFC connection is established between them and both devices start recording data from a pre-specified sensor.
Upon successful completion of the measurements, the two devices store the recorded data in a local database file, as shown in Figure~\ref{fig:Architecture}.

\begin{figure}[ht]
	\centering
	\includegraphics[scale=0.4]{images/Diagram.png}
	\caption{Architecture}
	\label{fig:Architecture}
\end{figure}

A more detailed view of the process is depicted in Figure~\ref{fig:diagram}.
Touching the two devices triggers the terminal application to send a message to the mobile device, listing the pre-defined sensor to be used in the current transaction on the terminal side and a transaction ID\@.
After the finalisation of the data transfer to the mobile device, both devices initiate the data recording process for the pre-selected sensor.
The recording process takes place for 500ms, as this is the maximum allowed time period in which a contactless transaction should complete, according to the \textit{MasterCard Contactless Performance Requirements} \cite{MasterCard2014}.
According to the same document, as of the beginning of 2016, the amount of time will be gradually reduced to 400ms.
For transport related transactions, the transaction time should not exceed 300ms \cite{transport300, VISAMobileTicketing2013}.
The design of the local application databases allows subtracting values captured after some certain time interval from a measurement, that can be used for analysis purposes in such scenarios.
After the completion of a measurement, the mobile device validates the data that were received from the terminal and returns a completion or rejection message accordingly, including the sensor that was used and the ID that was received from the terminal.
The terminal application can then ensure that it is in the same transaction as the mobile device, and if not, reject the measurement.
Finally, the terminal verifies the data received from the mobile device.
Upon validation, the devices save the measurements in their local database files.

\begin{figure}[ht]
	\centering
	\resizebox{\columnwidth}{!}{
		\begin{sequencediagram}

			\tikzstyle{inststyle}+=[rounded corners=3mm]
			\newthread{reader}{Terminal}
			\newinst[4]{card}{Mobile device}
			\begin{call}{reader}{1) sensor|transaction ID}{card}{2) sensor|transaction ID}
				\begin{callself}{reader}{recordSensor()}{}
					\postlevel
				\end{callself}
				\prelevel\prelevel\prelevel
				\begin{callself}{card}{recordSensor()}{}
					\postlevel
				\end{callself}
				\begin{callself}{card}{validateReceivedData()}{}
				\end{callself}
			\end{call}

			\begin{callself}{card}{saveMeasurement()}{}
			\end{callself}
			\prelevel\prelevel
			\begin{callself}{reader}{validateReceivedData()}{}
			\end{callself}
			\begin{callself}{reader}{saveMeasurement()}{}
			\end{callself}

		\end{sequencediagram}
	}
	\caption{Sensor recording}
	\label{fig:diagram}
\end{figure}

\subsection{Data Collection Framework}
In order to understand the variance between the environment and sensor-based proximity detection, the experiment took place in four different locations in the university: The lab, the cafeteria, the dining hall and the library.

In order to study how sensor measurements can be affected by user behaviour, a user-study was conducted in all locations excluding the lab, where 252 participants provided a variant number of transactions for each sensor.
%Figure~\ref{fig:Experiment} shows the setting of the experiment.

Four devices were used in the experiments, forming two sets of \textit{terminal-mobile device} pairs.
The first pair consisted of two Nexus 9 tablets.
The second pair consisted of two Android smartphones, a Nexus 5, acting as the terminal and a Samsung Galaxy S5 mini (SGS5 mini), acting as the mobile device.
Not all sensors were present on all devices.
The ones that were present on the tablets were tested on the first experimentation set, and the rest on the second.
Table~\ref{tab:availability} lists all the available sensors for each device, as well as which sensors were used on which set.
Sensors with technical limitations did not return any data, at least not in the 500ms timeframe, with the exception of Bluetooth, which returned data a very limited amount of times.
Two sensors, the humidity and the temperature sensors, are rare among Android devices and none of the devices used in the experiments include them, therefore they have been excluded from this study.

\begin{table}[ht]
	\centering
	\caption{Sensor availability}
	\label{tab:availability}
	\resizebox{\columnwidth}{!}{
		\begin{threeparttable}
			\begin{tabular}{@{}lcccc@{}}
				\toprule
				\multicolumn{1}{c}{\textbf{Sensors}} & \textbf{Tablet 1} & \textbf{Tablet 2} & \textbf{Nexus 5} & \textbf{SGS5 mini} \\ \midrule
				\rowcolor[HTML]{EFEFEF}
				\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}Tablet 1 $\rightarrow$ Tablet 2} \\
				\textbf{Accelerometer} & \cmark & \cmark & \cmark & \cmark \\
				\textbf{Bluetooth} & $\ast$ & $\ast$ & $\ast$ & $\ast$ \\
				\textbf{GRV$^\dag$} & \cmark & \cmark & $\ast$ & \cmark \\
				\textbf{GPS} & $\ast$ & $\ast$ & $\ast$ & $\ast$ \\
				\textbf{Gyroscope} & \cmark & \cmark & \cmark & \cmark \\
				\textbf{Magnetic Field} & \cmark & \cmark & \cmark & \cmark \\
				\textbf{Network Location} & \cmark & \cmark & \cmark & \cmark \\
				\textbf{Pressure} & \cmark & \cmark & \cmark & \xmark \\
				\textbf{Rotation Vector} & \cmark & \cmark & $\ast$ & \cmark \\
				\textbf{Sound} & \cmark & \cmark & \cmark & \cmark \\
				\textbf{WiFi} & $\ast$ & $\ast$ & $\ast$ & $\ast$ \\
				\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}SGS5 mini $\rightarrow$ Nexus 5} \\
				\textbf{Gravity} & $\circ$ & $\circ$ & \cmark & \cmark \\
				\textbf{Light} & $\ast$ & $\ast$ & \cmark & \cmark \\
				\textbf{Linear Acceleration} & $\circ$ & $\circ$ & \cmark & \cmark \\
				\textbf{Proximity} & \xmark & \xmark & \cmark & \cmark \\
				\multicolumn{5}{c}{\cellcolor[HTML]{EFEFEF}Unsupported} \\
				\textbf{Humidity} & \xmark & \xmark & \xmark & \xmark \\
				\textbf{Temperature} & \xmark & \xmark & \xmark & \xmark \\ \bottomrule
			\end{tabular}

			\begin{tablenotes}
			\item\cmark: Working properly.
				\xmark: Not present on device.
				$\ast$: Technical limitations.\\
				$\circ$: Only returning \textit{0s}.
			\item[\dag] Geomagnetic Rotation Vector
			\end{tablenotes}
		\end{threeparttable}

	}
\end{table}

Total of 1000 measurements were recorded for each sensor in order to be used in the analysis phase.
700 measurements for each sensor took place in the lab and 100 on each of the remaining locations.
With the exception of the sound sensor, sensors typically return an object that contains the captured data every time these change, or when they are returned by the operating system.
In the case of the sound sensor, the data returned from the microphone was written directly in an audio file.

Each measurement for each sensor created one database record.
Data recorded from a sensor were stored in the database, in XML form.
Each time sensor values were returned, a new child element was created, containing the sequence ID of the measurement, the timestamp, setting the time that the recording was initiated to time zero, and the returned sensor data.
Listing~\ref{lst:xml} shows a sample record, as saved in XML form.
The subchild elements were saved in generic format \textit{(ex.\ data0, data1, etc.)} for convenience reasons, and later assigned to their actual units during the analysis phase, according to the Android documentation~\cite{sensorUnits}.
Details for each sensor can be found in Appendix~\ref{sec:AmbientSensors}.

\begin{lstlisting}[style=listXML, caption={Sample XML}, label={lst:xml}]
<?xml version="1.0" encoding="UTF-8"?>
<measurements>
	....
	<measurement>
		<id>6</id>
		<timestamp>60</timestamp>
		<data0>-0.32935655</data0>
		<data1>6.2396774</data1>
		<data2>-7.558329</data2>
	</measurement>
	....
</measurements>
\end{lstlisting}

The sequence ID of each measurement, the actual date and time that the measurement was initiated, the pre-defined location in which it was captured and the transaction ID that was sent from the terminal to the mobile device in the beginning of the transaction were also stored in the database.

The transaction ID is a random 7-byte string generated by the terminal, and is used for assisting the linkage of transactions stored in the two devices of the set, in case some measurements have not been stored on the terminal side.
This typically occurs because the applications are built to reject any recorded data in case the NFC connection is lost.
In some rare occasions the connection is disrupted when the mobile device has already sent the reply to the terminal (message 2 in Figure~\ref{fig:diagram}), but the last has not yet received it.
Using the transaction ID, such transactions can be detected and excluded from the analysis phase, when not required.

%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=0.75\columnwidth]{images/experiment.png}
%	\caption{Experiment}
%	\label{fig:Experiment}
%\end{figure}

In the end of the experiment, the databases were extracted from the devices and transfered to the machine that runs the analysis software via USB.


==> sections/framework_part2.tex <==
\subsection{Data Analysis and Evaluation Criteria}
\label{sec:DataAnalysisandEvaluationCriteria}

After retrieving the databases for the reader and the card, the set of all transactions, $T$, was produced using the shared IDs generated during data collection.  Each transaction, therefore, may be thought of as the set of reader and card values, $R_{i}$ and $C_{i}$, with the same shared ID, i.e. $T_{i} = (R_{i}, C_{i})$.  A Python application was developed for analysing the transaction measurements produced from the reader and card applications, employing the SciPy library \cite{scipy} for numerical computation.

To compare $(R_{i}, C_{i})$, we measure the similarity distance between the two, which was measured differently according to sensor type. 
For network location, this was calculated using the Haversine formula (Eq.\ \ref{haversineeq}), which measures the geographic distance between two latitude and longitude pairs, $\{(\phi_1, \lambda_1), (\phi_2, \lambda_2)\}$.
With sound, we use the sum of the absolute values of the frequencies of the recorded sound, in 2ms intervals.
For all other sensor types, similarity was measured using the \emph{mean absolute error} (MAE, Eq.\ \ref{aadeq}) and \emph{correlation coefficient} (Eq.\ \ref{correq}), as used in \cite{merh2014}, between the signals of $R_{i}$ and $C_{i}$, with each containing $N$ measurements.  Certain sensors -- the accelerometer, gyroscope, magnetic field, rotation vector and GRV sensors -- produce a vector of values comprising $x$, $y$ and $z$ components.  In these instances, the vector magnitude (Eq.\ \ref{mageq}) was used as a general-purpose method for producing a single, combined value prior to computing the MAE and correlation coefficient.

%Sound equation
% Equations.  Please feel free to clean these up...
\begin{equation}
2r\footnote{$r$ represents the radius of Earth: 6371km} \arcsin  \left(\sqrt{\sin^2\frac{\phi_2 - \phi_1}{2}
+ \cos{\phi_1} \cos{\phi_2}\sin^2\frac{\lambda_2 - \lambda_1}{2}}\right)
\label{haversineeq}
\end{equation}

\begin{equation}
M = \sqrt{x^{2} + y^{2} + z^{2}}
\label{mageq}
\end{equation}

\begin{equation}
MAE(R_{i}, C_{i}) = \frac{1}{N}\sum_{j=0}^{N} | R_{i,j} - C_{i,j} |
\label{aadeq}
\end{equation}

\begin{equation}
corr(R_{i}, C_{i}) = \frac{covariance(R_{i}, C_{i})}{\sigma_{R_{i}} \cdot \sigma_{C_{i}}}
\label{correq}
\end{equation}


==> sections/introduction.tex <==
\section{Introduction}
Contactless smart cards are being deployed in multitude of application areas ranging from banking, transport and access control applications \cite{markantonakis2013secure}. The awareness and acceptance of contactless cards is increasing, especially in the banking sector \cite{UKCardsAnnualRep2015a}. As the acceptance of the contactless cards growing, the mobile (contactless) payments gaining acceptance -- especially ``among early adopters and young age groups" \cite{UKCardsPayment2015a}. In mobile (contactless) payments, the Near Field Communication (NFC) provides the platform to emulate a contactless smart card. It is expected that five percent of 600-650 million NFC enabled mobile phones will be used at least once a month in 2015 to make a contactless payment \cite{Deloitte2015}. Therefore, we can safely assume that mobile payments are going to be a big payment instrument in future, may be even potentially overtaking the contactless smart cards. Although the above discussion is limited to financial industry; however, the similar trends are also seen other domains where contactless smart cards are deployed \cite{VeriFone2010}.

Contactless smart cards are susceptible to relay attacks \cite{Hancke2009615,Hancke06,kfir2005picking} and so the NFC enabled mobile phones \cite{FrancisHMM11,FrancisHMM10,madlmayr2008nfc,6482441}. A relay attack is a passive man-in-the-middle attack in which an attacker extends the distance between the genuine terminal (point-of-service) and genuine contactless smart card (or an NFC enabled mobile phone). This attack can enable a malicious user to access services that the genuine user is eligible, for example, paying for some goods or accessing a building that uses digital access controls. 

It is challenging to gauge the actual fraudulent activities targeted as using relay attacks on contactless tokens (smart card and NFC mobile phones). However, there is evidence that academic work dealing with attacks on smart cards were adopted by the real-world criminals \cite{Ferradi2015}. In the contactless smart card domain, a potential and effective countermeasures has been the distance bounding protocols \cite{hancke2005rfid,trujillo2010poulidor}. To provide potential countermeasures to the NFC enabled mobile phones, in academic literature ambient sensors are being put as an effective countermeasures (section \ref{sec:AmbientSensorDeploymetinMobilePayment}). In this paper, we took the ambient sensors available in the Google Android devices and build a test-bed environment (section \ref{sec:FrameworkforEvaluationofAmbientSensorsEffectiveness}) to test their effectiveness as a anti-relay mechanism for NFC based transactions (section \ref{sec:AmbientSensorEvaluation}). We also evaluate individual sensors on their technical feasibility and challenges that we had to overcome to implement them (section \ref{sec:ExperimentationandChallenges}).The main objective of the paper is to provide an empirical foundation to the analysis of ambient sensor's validity as a anti-relay mechanism (section \ref{AntiRelayMechanismandAmbientSensorsTheVerdict}). 

In this paper, we keep on referring to contactless mobile payments as it is potentially one of the deployment envionrment that can attract lot of malicious attention due to potential financial gains. However, the discussion in this paper is also valid of the deployment of contactless mobile phone based solution in any other domain like transport or access control etc.

\subsection{Contribution of the Paper}
There are three main contributions of the paper:

\begin{enumerate}
\item A test-bed architecture and implementation that can be used to evaluate different sensors on the Google Android devices.
\item A data analysis framework and implementation on how to evaluate the sensor measurements.
\item Empirical evaluation of ambient sensor's effectiveness as a anti-relay mechanism. This evaluation provides a factual foundation to decide which sensors to deploy in a target environment.
\end{enumerate}

Also the implementation of test-bed, and data analysis along with collected data sets are being made available online from \url{http://anonymised}





==> sections/verdict.tex <==
\section{Outcome and What's Next}
\label{AntiRelayMechanismandAmbientSensorsTheVerdict}
%\todo[linecolor=green!90!white, backgroundcolor=purple!20!white,
% bordercolor=red, inline]{Mainly written by Raja... Iakovos \& Carlton to assist}

The data collection and analysis presented in the previous section provides us an empirical evidence to evaluate the applicability of mobile sensors as a proximity detection mechanism for NFC mobile phones based services. As discussed in the previous section, the higher the threshold for the optimum EER it is more likely that an attack might pass through undetected. Based on the empirical data and the analysis carried out it is difficult to recommend any of the sensors (individually) for a high security deployment application like banking. These sensors might be valid for access control but we recommended a through analysis should be carried out of the sensors and their performance in the deployment environment before rolling them out. 

On potential reason that other research carried out in this domain has achieved different results from us might be to do with larger sample duration and limited field tests. The limited imposed during our experiments were inline with the transaction requirement of an EMV application (i.e. 500 milliseconds). Whereas, one of the biggest application areas along with banking where contactless smart cards are deployed is transport. In the transport application, the recommended duration for a transactions is much lower, in the range of 300 to 400 milliseconds. Therefore, imposing the limit of 500 millisecond in our experiments was based on the upper bound of the current recommendations from two of the application areas where most of the contactless mobile phones might be utilised. 

During the experimentation, we realised that sensors and the associated platform might not be matured and standardised at this point of time for their field deployments as proximity detection mechanisms in NFC mobile phones. Each manufacturer might develop their sensors different, the mobile platform's sensor data polling mechanism might be effective by other tasks running simultaneously, and sensor measurement frequency rate might be different between mobile handset manufacturer. We consider that mobile sensors have to go a long way before they can reach the necessary granularity of measurements, inter-operable and supported specifications, and effectiveness to prevent rely-attacks. 

From our experimentation, we can  claim with a high degree of confidence that mobile sensors at least in their current state in mainstream Google Android devices are not suitable for anti-relay mechanism. Especially in the case of high security requirement applications like banking, transport, and access-control at highly sensitive sites. 

As part of the future research direction, we will investigate:

\begin{itemize}
\item Collect a large data set of relay-attacks using these sensors for evaluation, providing how a relay-attack in the field would be represented in the sensor measurements.
\item Can we simultaneously measures multiple sensors within the transaction time duration? If so will it reduce the risk associated with the these sensors individually. 
\item Combining sensor measurements with time slices -- only one sensor is measured as a time but over the duration of the measurement multiple sensors are used.  
\item Can a localised sensor training and operational deployment would be feasible? Will it improves the sensor's success rate if localised analysis is preformed. 
\end{itemize}


